Full and Reduced Order Model Consistency of the Nonlinearity Discretization in Incompressible Flows

We investigate both theoretically and numerically the consistency between the nonlinear discretization in full order models (FOMs) and reduced order models (ROMs) for incompressible flows. To this end, we consider two cases: (i) FOM-ROM consistency, i.e., when we use the same nonlinearity discretization in the FOM and ROM; and (ii) FOM-ROM inconsistency, i.e., when we use different nonlinearity discretizations in the FOM and ROM. Analytically, we prove that while the FOM-ROM consistency yields optimal error bounds, FOM-ROM inconsistency yields additional terms dependent on the FOM divergence error, which prevent the ROM from recovering the FOM as the number of modes increases. Computationally, we consider channel flow around a cylinder and Kelvin-Helmholtz instability, and show that FOM-ROM consistency yields significantly more accurate results than FOM-ROM inconsistency.

==> notation.tex <==
\newcommand{\EX}{{\Bbb{E}}}
\newcommand{\PX}{{\Bbb{P}}}

% \left \right 
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}
\newcommand{\lbr}{\left\{}
\newcommand{\rbr}{\right\}}
\newcommand{\lnorm}{\left\|}
\newcommand{\rnorm}{\right\|}




\def\PP{{{\rm l}\kern - .15em {\rm P} }}
\def\PN2{{\PP_{N}-\PP_{N-2}}}

\newcommand{\erf}[1]{\mbox{erf}\left(#1\right)}

% math symbols
\newcommand{\D}{\mathbbm{D}}
\newcommand{\I}{\mathbbm{I}}
\newcommand{\N}{\mathbbm{N}}
\newcommand{\R}{\mathbbm{R}}
\newcommand{\Z}{\mathbbm{Z}}

% calligraphic letters
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}


% boldface Greek letters
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bLambdar}{\boldsymbol{\Lambda}_r}
\newcommand{\bLambdarL}{\boldsymbol{\Lambda}_r^{L^2}}
\newcommand{\bLambdarH}{\boldsymbol{\Lambda}_r^{H^1}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPhir}{\boldsymbol{\Phi}_r}
\newcommand{\bphi}{\boldsymbol{\varphi}}
\newcommand{\bphir}{\boldsymbol{\varphi}_r}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\btau}{\boldsymbol{\tau}}

% boldface letters
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bas}{{\boldsymbol a}^{snap}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bFF}{{\boldsymbol F}}
\newcommand{\bG}{{\boldsymbol G}}
\newcommand{\bGs}{{\boldsymbol G}^{snap}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bq}{{\boldsymbol q}}
\newcommand{\bqs}{{\boldsymbol q}^{snap}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bur}{{\boldsymbol{u}}_r}
\newcommand{\bUr}{{\boldsymbol{U}}_r}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bvr}{{\boldsymbol{v}}_r}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bwr}{{\boldsymbol{w}}_r}
\newcommand{\bWr}{{\boldsymbol{W}}_r}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bXh}{{\bf X}^h}
\newcommand{\bXr}{{\bf X}^r}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bz}{\boldsymbol{z}}

% tilde letters
\newcommand{\tA}{\tilde{A}}
\newcommand{\tB}{\widetilde{B}}
\newcommand{\tC}{\widetilde{C}}


% overline letters
\newcommand{\oa}{\overline{a}}
\newcommand{\oA}{\overline{A}}
\newcommand{\oc}{\overline{c}}
\newcommand{\obc}{\overline{\boldsymbol c}}
\newcommand{\op}{\overline{p}}
\newcommand{\oU}{\overline{U}}
\newcommand{\obu}{\overline{\boldsymbol u}}
\newcommand{\obU}{\overline{\boldsymbol U}}
\newcommand{\obur}{\overline{\boldsymbol{u}_r}}
\newcommand{\obUr}{\overline{\boldsymbol{U}_r}}
\newcommand{\obv}{\overline{\boldsymbol v}}
\newcommand{\obx}{\overline{\boldsymbol x}}
\newcommand{\ob}[1]{\overline{\boldsymbol{#1}}}
\newcommand{\orr}[1]{\overline{#1}^r}
\newcommand{\obr}[1]{\overline{\boldsymbol{#1}}^r}
\newcommand{\oh}[1]{\overline{#1}^h}
\newcommand{\obh}[1]{\overline{\boldsymbol{#1}}^h}

% POD notation
\newcommand{\as}{a^{snap}}
\newcommand{\CinvNabla}{C_{inv}^{\nabla}(r)}
\newcommand{\CinvDelta}{C_{inv}^{\Delta}(r)}
\newcommand{\Deltar}{\Delta_r}
\newcommand{\Gs}{G^{snap}}
\newcommand{\ct}{\bu_h^{avg}}



\newcommand{\bus}{{\bf u}^*}
\newcommand{\By}{\mathcal B(\by)}
\newcommand{\eci}[1]{\mathcal E_{#1}}
\newcommand{\dpyi}[1]{\delta_{#1}^+(\by)}
\newcommand{\dmyi}[1]{\delta_{#1}^-(\by)}
\newcommand{\cA}{{\mathcal A(\by)}}
\newcommand{\dyi}[1]{\delta_{#1}(\by)}
\newcommand{\cG}{{\mathcal G(\bx,\by)}}
\newcommand{\cGi}[1]{{\mathcal G_{#1}(\bx,\by)}}
\newcommand{\pti}{\partial_i}
\newcommand{\ptii}[1]{\partial_{#1}}
\newcommand{\vertiii}[1]{{|\!|\!| #1 |\!|\!|}}

% fractions
\newcommand{\half}{\frac{1}{2}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% colors
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\definecolor{vargreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\green}[1]{{\color{vargreen} #1}}

\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\inserted}[1]{\blue{#1}}
\newcommand{\deleted}[1]{{}}%\color{red}{#1}}}
%\newcommand{\comment}[1]{{\color{cyan}#1}}


% comments
\newcommand{\TI}[1]{{\color{blue}TI: #1}}
\newcommand{\DRW}[1]{{\color{vargreen}DRW: #1}}
\newcommand{\ZW}[1]{{\color{red}ZW: #1}}
\newcommand{\XX}[1]{{\color{brown}XX: #1}}
\newcommand{\CM}[1]{{\color{purple}CM: #1}}





